Kitchen Artist: Precise Control of Liquid Dispensing for Gourmet Plating

Manipulating liquid is widely required for many tasks, especially in cooking. A common way to address this is extruding viscous liquid from a squeeze bottle. In this work, our goal is to create a sauce plating robot, which requires precise control of the thickness of squeezed liquids on a surface. Different liquids demand different manipulation policies. We command the robot to tilt the container and monitor the liquid response using a force sensor to identify liquid properties. Based on the liquid properties, we predict the liquid behavior with fixed squeezing motions in a data-driven way and calculate the required drawing speed for the desired stroke size. This open-loop system works effectively even without sensor feedback. Our experiments demonstrate accurate stroke size control across different liquids and fill levels. We show that understanding liquid properties can facilitate effective liquid manipulation. More importantly, our dish garnishing robot has a wide range of applications and holds significant commercialization potential.

==> Archived/01Introduction.tex <==
\section{Introduction} \label{introduction}

Liquids are common across households and industries. An autonomous robot in these environments must be able to manipulate and distribute liquids. This involves various common tasks like applying sauces on hotdogs, filling cups with juice, or precisely dispensing chemicals to create mixtures. While many works have explored liquid pouring for robots \cite{Matl2019}, tasks like dispensing viscous liquids or dispensing precise small amounts often rely on squeezing actions. For example, distributing salad dressing, garnishing dishes with sauces, or applying sunscreen requires squeezing motions. Despite its significance, the squeezing actions remain relatively unexplored in the field of robotics.

\begin{comment}
問題定義
1. 一個重要擠液體的目標是控制擠出線條的粗細度（擺盤）或每單位長度的體積（沙拉醬）
2. 我們的目標是讓機器人能在任何液體任何體積下都能達到這些目標
3. 最終，我們希望設計一套系統用任何醬料擠出任何線條藝術（如圖一）
4. 為了控制線條大小，不失普遍性，我們固定手指擠的方式，只控制畫的速度

\end{comment}

An important goal for liquid squeezing is to control the width (e.g., dish garnishing) or volume-per-length (e.g., distributing salad dressing) of the liquid stream on a surface. We aim for the robot to achieve this with diverse liquid types and quantities. Eventually, we want to design a system capable of producing line arts (Figure \ref{fig:fig1}) using different sauce types and fill levels. To control its stroke, without loss of generality, we employ a fixed finger squeezing motion during dispensing and only control the nozzle's horizontal movement speed (drawing speed).

\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{Figures/Fig1.png}
\caption{We develop a liquid dispensing system capable of garnishing dishes with unseen sauces. The robot adjusts its dispensing strategy based on the sauce properties explored through a rotating action.}
\label{fig:fig1}
\end{figure}

\begin{comment}
為何困難
1. 雖然加裝感測器監控線條粗細或單位長度體積然後反饋控制畫的速度很直覺，這方法有實務上的困難
2. 視覺監控線條狀態只在無遮蔽且液體不透明而且不流動情況下可行，而且視覺延遲會造成反饋失準
3. 手腕的力感測器不可行因為誤差以及手臂移動時的馬達震動足以蓋過微量液重改變導致的力變化
4. 我們的方法捨棄即時反饋並採取開環控制
\end{comment}

Although it seems intuitive to attach sensors for real-time measurement of liquid stream thickness or volume-per-length and feedback controlling the drawing speed, practical challenges arise. For example, visually monitoring the stroke is limited to scenarios where the dispensed liquid is neither occluded nor transparent and remains still. Similarly, monitoring the dispensed quantity using a force sensor on the robot's wrist is challenging due to sensor noise and motor vibrations, which can mask the subtle measured weight loss caused by the dispensed liquid. Therefore, our approach embraces open-loop control, foregoing real-time feedback.

\begin{comment}
我們的解法
我們開發了一種方法在擠之前就算出每瞬間手臂需要移動的速度以畫出我們想要的線條。
具體而言，我們需要預測在我們的固定擠法下留宿隨時間的變化以及液體在平面上的堆積模式。
這些都與液體的黏度與瓶內容量高度相關，於是我們採用兩階段的方法：探索階段與擠的階段。
1. 探索階段，機器人會轉動瓶子並用力受器感受液體反應。液體的反應會包含瓶中液體的資訊，我們訓練一個神經網路來預測這種液體及量在我們固定的擠法下的Flow Rate Curve以及Stacking Pattern。
2. 一般來說，當轉動瓶子時，液體感覺比較容易流動，則可以預測液體在擠的時候會出來得比較快以及在平面上比較容易塌陷以形成很寬的線條。
3. 擠的階段，藉由預測的flow rate curve and stacking pattern，機器人算出擠嘴每瞬間需要移動的速度來控制volume-per-length以及粗細度。
4. 整個擠的階段是開環的，沒有任何sensor feedback。
\end{comment}

In this work, we present a method to calculate drawing speed for achieving desired strokes before dispensing. In particular, we predict how the flow rate changes over time (\textit{flow rate curve}) and how the liquid stacks to form strokes on a surface (\textit{stacking pattern curve}). These are determined by the liquid's viscosity and the bottle's fill level. To address this, we propose a two-phase approach: an exploration phase and a dispensing phase. In the exploration phase, the robot rotates the bottle and uses a force-torque sensor (F/T sensor) to sense the liquid's responses, providing information about liquid properties. We leverage this information and train a neural network that predicts the flow rate curve and stacking pattern curve. A more fluid-like liquid movement suggests lower viscosity, potentially leading to a higher flow rate during dispensing and wider strokes due to collapse. In the dispensing phase, the predicted flow rate curve and stacking pattern curve determine the drawing speed for controlling stream thickness or volume-per-length. This phase operates in an open-loop manner.

\begin{comment}
貢獻與結果
1. 據我們所知，我們是第一篇研究機器人擠液體的論文。
2. 我們的核心貢獻有兩個: 
    對於未知的液體與未知的量，我們能藉由探索來直接預測擠他的時候的fow rate curve以及stacking pattern。
    一個擠液體的系統，在完全無反饋的情況下，我們能對未知的液體與量控制擠出的粗細度或volume-per-length。並以此讓機器人可以用任何醬料畫任何線條圖。
3. 藉由實驗，我們證明對於未知的液體與量，我們能控制擠出粗細度在誤差X%，volume-per-length在誤差Y%。
\end{comment}

\textbf{Contributions:} To the best of our knowledge, we are the first to study liquid squeezing with robots. Our research introduces two key contributions. First, we utilize an exploratory motion to predict the flow rate curve and stacking pattern curve of unseen liquids and uncertain fill levels. Second, using the predicted curves, we design a liquid dispensing system that can control stream thickness and volume-per-length without any real-time sensor feedback. Additionally, we've developed a robot system capable of creating line art using various sauces. We show our method outperforms the baselines. With unseen liquids and unknown fill levels, our approach can control the stream thickness within $29\%$ error.

==> Archived/03Method.tex <==
\section{Method} \label{method}

\begin{figure*}
\centering
\includegraphics[width=0.98\linewidth]{Figures/Fig2.jpg}
\caption{Pipeline of SqueezeBot. The robot follows these steps to achieve its liquid dispensing goals: (1) Rotate the bottle $90$ degrees, pause for 10 seconds, and record haptic signals with a wrist-mounted F/T sensor. We process this signal to obtain the liquid property feature. (2) The feature is fed into an MLP to predict the dispense curve (total dispensed amount over time) and another MLP to predict the stacking pattern curve (volume-per-length for various stream thickness levels). (3) We utilize the predicted curves to guide the dispensing phase. The squeezing motion in the dispensing phase is fixed. We control the total dispensed volume by adjusting the dispense duration and stream thickness by controlling the nozzle speed.}
\label{fig:fig2}
\end{figure*}

\begin{comment}
簡介
1. 我們的目標是在瓶內裝有任何液體以及任何量的清況下能夠控制擠出的線條粗細度以及單位長度的體積
2. 我們選擇固定擠法而透過控制手臂的移動速度來控制擠出的線條
3. 
2. 我們的方法包含兩階段
3. 探索階段的目的是透過晃動液體來獲取液體的資訊，並直接預測擠這種液體的Dispense Curve。
4. 在擠的階段，藉由預測的Dispense Cruve，我們控制擠的時長來改變擠出總量，控制擠嘴移動速度來改變擠出的粗細。
5. 整個過程見Figure X.
\end{comment}
In this work, we aim to control the dispensed volume and stream thickness when dealing with different liquids and bottle fill levels. We employ a two-phase approach: exploration and dispensing. During the exploration phase, we perturb the bottle to gather liquid property information. This information allows us to predict the dispense curve (how dispensed volume changes over time) with our fixed squeezing motion. In the dispensing phase, we use this predicted curve to guide either the squeezing duration for total volume control or the nozzle's speed for stream thickness control. The pipeline is shown in Figure \ref{fig:fig2}.

\subsection{Haptic Exploration and Pre-processing}
\begin{comment}
探索階段
1. 在探索階段，我們透過轉動瓶子並紀錄手腕感受到的力來取得瓶內液體的資訊，包含著黏滯力以及總量
2. 我們選擇花一秒轉動瓶子九十度然後等待十秒，過程中液體在瓶內流動的資訊會被手腕力測器記錄下來
3. 根據其他研究，轉動中的力變化可以提供液體總量訊息，轉動後液體震盪的力變化可以提共液體黏滯力的訊息。
\end{comment}

In the exploration phase, the robot rotates the bottle to acquire information about the contained liquid's properties, such as viscosity and fill level. By rotating the bottle for $90$ degrees in one second, followed by a $10$-second pause, the robot's wrist-mounted F/T sensor records haptic signals (torque in the wrist's rotation direction) generated by the liquid's movement. According to [Matl], haptic signals during rotation provide information about fill level, while post-rotation torque changes indicate liquid viscosity.

\begin{comment}
訊號處理
1. 我們單獨處理轉動中及轉動後的力訊號並整合成一個feature以預測Dispense Curve
2. 我們均勻採樣轉動中的力訊號
3. 我們抽取轉動後力訊號的頻譜，然後取得0.1 hz 到2.5 hz的資訊
4. 最後我們把兩個feature以及瓶子與液體總重的訊息拼接成一個X dim的feature
\end{comment}

We independently process the haptic signals recorded during and after the rotation, and subsequently concatenate them to create the liquid property feature. We downsample the torque signals obtained during the one-second rotation at intervals of $0.1$ seconds. For the torque signal collected during the subsequent free oscillation period, we extract its frequency domain within the range of $0.1$ Hz to $2.5$ Hz. These two features are concatenated with the total weight of the bottle and its liquid contents, resulting in a $33$ dimensional liquid property feature.

\subsection{Inferring the Dispense Curve}
\begin{comment}
1. 擠的時候的Dispense Curve跟液體性質以及擠壓動作相關。
2. 為了簡化問題，我們採取一種固定的擠壓動作(Figure X)，也就是先快速的擠到一定程度再慢慢擠。
3. 如此一來，Dispense Curve只與液體性質相關。
\end{comment}

The dispense curve is determined by both the liquid's property and the squeezing motion. To simplify the problem, we utilize a fixed gripper closing motion (Figure 4): a $2$-second rapid squeeze followed by a $15$-second gradual squeeze. With this fixed squeezing motion, the dispense curve can be entirely determined by the liquid properties, allowing it to be deduced solely from the liquid property feature developed during the exploration phase.

\begin{comment}
1. 我們訓練一個MLP模型以探索階段採到的液體feature為input來預測Dispense Curve的微分也就是流速曲線。
2. 之所以沒有explicitly的先用液體feature預測液體黏至力以及總量，然後再預測流速曲線是因為也許有其他液體性質可以影響流速曲線。
3. 具體來說，我們用流速曲線上均勻的二十個點來參數化他，而MLP的目標就是精準預測這二十個值。
4. 整個訓練流程採用supervised learning，資料採集以及訓練參數請見下章。
5. 測試時，我們會用spline把二十個預測的點接起來重現平滑的流速曲線，然後積分以獲得Dispense Curve。
6. Figure X呈現了不同液體其對應的力訊號，Dispense Curve，以及流速曲線。
\end{comment}

Instead of directly predicting the dispense curve, we train an MLP model taking the liquid property feature as input to predict the dispense curve's derivative. This derivative is referred to as the "flow rate curve," which specifies the flow rate changes over time during squeezing. We avoid explicit predictions for liquid viscosity and filling level because other liquid properties encapsulated within the liquid property feature may affect the flow rate curve. We parameterize the flow rate curve by the flow rate values at each second, and the MLP's objective is to predict these values accurately. The model is trained in a supervised fashion (see Section \ref{experiment_setup} for details). During testing, we connect the predicted flow rate values using splines to reconstruct the smooth flow rate curve, which is then integrated to obtain the predicted dispense curve. Figure 3 shows the torque data collected during the exploration phase, the dispense curve, and the flow rate curve for various liquids and filling levels.

\subsection{Control Total Dispensed Amount}

\begin{comment}
1. 擠東西最常見的目標是控制擠出來的總量，例如擠油醋醬到沙拉裡。
2. 雖然最直接的方式是直接測量擠出來的總量，但如introduction所說，這通常有實務上困難。
3. 透過探索階段預測的Dispense Curve，我們可以計算甚麼時候放開可以擠到我們想要的量，整個過程不需要真實測量擠出的量。
\end{comment}

The most common goal of squeezing is to control the overall amount dispensed. For example, the desire to control the quantity of salad dressing dispensed onto a salad. While the most intuitive approach involves employing sensors to directly sense the total amount dispensed, as stated in Section \ref{introduction}, this is often practically challenging. By utilizing the predicted dispense curve in the exploration phase, our approach can determine when to stop squeezing to achieve our desired dispensed quantity. In the dispensing phase, we squeeze until such time.

\subsection{Control the Stream Thickness}

\begin{comment}
1. 我們也希望能夠控制擠出來液體流的粗細程度，例如可以用於擺盤(Figure X)。
2. 藉由探索階段預測的Flow Rate Curve，我們可以預測每時刻的液體流速。
3. 當我們想要擠出一條每公分X ml而當前流速是v ml/s，則擠嘴橫向移動的速度需要是v/X cm/s。
4. 然而如果我們想要控制的是液體幾何上的粗細，我們需要知道這種液體的堆積曲線:在線上每公分的體積與線條粗細的關係(Figure X)。
5. 這個關係與液體黏滯度直接相關，假設液體很黏，即使每公分體積很大，液體也不容易塌陷，因此會呈現比較細。
\end{comment}

We also want to enable the robot to control the stream thickness when squeezed on a flat surface, which is required for dish garnishing (Figure \ref{fig:fig1}). Using the flow rate curve predicted in the exploration phase, we can predict the liquid flow rate at any moment. To achieve a desired stream with a volume-per-length of V ml/cm while the current flow rate is predicted as Q ml/s, we simply adjust the nozzle moving speed to Q/V cm/s. However, to control the geometric stream thickness, we need to know the liquid's \textit{stacking pattern curve}. The stacking pattern curve shows how the thickness of the stream varies at different volume-per-length values (Figure 3). The curve is governed by the liquid viscosity. Viscous liquids tend to create a thinner stream for a fixed volume-per-length, as it is more prone to collapsing.

\begin{comment}
1. 我們訓練一個MLP模型以探索階段採到的液體feature為input來預測液體的堆積曲線。
2. 我們用五個堆積曲線上均勻地點來參數話他，而MLP就是要精準預測這五個值。
3. 測試時，我們會用spline把這五個點連起來重現平滑的堆積曲線。
4. 於是當我們想要擠出一條粗x mm的線時，我們可以透過預測的堆積曲線來估計每公分需要擠多少體積的液體。
5. 然後透過Flow rate curve預測的當前流速來計算擠嘴橫向移動的速度並執行。
\end{comment}

We train an MLP model taking the liquid property feature as input to predict the stacking pattern curve of the liquid. To parameterize this curve, we use ten thickness values ranging from 5mm to 20mm, representing ten key points on the curve. The MLP will predict the volume-per-length of these ten points. During testing, we connect the predicted points with splines to reconstruct the smooth stacking pattern curve. When we want to squeeze a line with the desired thickness, we use the predicted curve to estimate the desired volume-per-length of the stream. Subsequently, we calculate the required nozzle moving speed based on the predicted flow rate at that particular moment.
